Physics-Guided Sequence-Based Generative Framework for Acoustic Metamaterial Inverse Design

Acoustic metamaterial (AMM) inverse design is particularly challenging for broadband target responses due to acoustic dispersion: a structure that matches the desired response at one frequency may deviate at others, and modifying geometry to improve one sub-band often perturbs neighboring sub-bands. Yet existing broadband inverse-design approaches are either constrained by predefined templates, or rely on image representations that fail to preserve the geometric precision and structural connectivity required by acoustic structures. We present MetaSeq, a physics-guided, sequence-based generative framework for acoustic metamaterial inverse design. At its core, MetaSeq introduces a language that represents each AMM as a structured sequence, rather than as a pixel grid or fixed template. This representation preserves precise geometry, explicitly encodes connectivity, and casts inverse design as a sequence-to-sequence task from target response to structure sequence. MetaSeq further constructs a balanced, high-fidelity dataset with efficient calibration and complexity-based sampling. To address the one-to-many nature of inverse design, MetaSeq combines supervised pretraining with reinforcement learning fine-tuning guided by a physics-based solver and validity checker. Extensive evaluations against COMSOL and five baselines show that MetaSeq reduces response error by 45% over the best baseline.

==> background.tex <==
% !TEX root = main.tex
\section{Background}
\subsection{Acoustic Metamaterials}
\sssec{Acoustic Metamaterial.}

\sssec{Acoustic Metasurface.} Acoustic metasurfaces (AMS) are structures capable of manipulating sound wavefronts with sub-wavelength resolution. The macroscopic behavior of an AMS is governed by the Generalized Snell's Law (GSL)~\cite{}, which relates the angle of reflection or transmission to the gradient of the phase discontinuity along the interface:
\begin{equation}
	\sin(\theta_t) - \sin(\theta_i) = \frac{c}{2\pi f} \frac{d\phi(x)}{dx}
\end{equation}
where $\theta_i$ and $\theta_t$ are the incident and transmitted angles, $c$ is the sound speed, $f$ is the frequency, and $\phi(x)$ is the spatially varying phase profile provided by the metasurface.

To realize specific macroscopic functions, including beam steering~\cite{} and acoustic focusing~\cite{}, one must first determine the ideal modulation profiles. For instance, focusing a plane wave to a point at focal length $F$ requires a phase distribution defined by $\phi(x) = \frac{2\pi f}{c} (\sqrt{x^2 + F^2} - F)$. While the phase profile $\phi(x)$ dictates the wavefront direction, the amplitude profile $A(x)$ is equally critical for ensuring high transmission efficiency. In practical implementations, these continuous profiles are discretized into an array of sub-wavelength unit cells located at positions $x_i$. Individual unit cells are required to independently modulate both the phase shift $\phi(x_i)$ and the transmission $T(x_i)$ of the incident wave. 

Consequently, one fundamental task for designing an AMS is to design physical unit cell structures that exhibit the precise target acoustic response in terms of both phase delay and transmission efficiency. However, the rapid expansion of AMS into broadband applications such as achromatic focusing and wideband noise absorption has significantly escalated this design challenge. This difficulty stems from the frequency-dependent dispersion~\cite{} of acoustic structures, which complicates the mapping between geometry and broadband response.

<<<<<<< HEAD
\subsection{Physical Acoustic Solver}\label{sec:solver}
Conventional acoustic response computation relies on finite-element method (FEM) simulations, which are accurate but expensive (often minutes per sample). To scale dataset construction,  we introduce an equivalent transmission lines-based solver that predicts spectral responses in milliseconds to achieve rapid dataset construction. 

=======
\subsection{Modeling Unit Cell Structure}\label{sec:solver}
>>>>>>> 49294a80e92cbd25c5b1529c159ff831200efa5e
The core of \sysname is an automated pipeline that translates geometric designs into rapid spectral predictions by treating the unit cell as a structural sequence. In this section, we introduce this process for transmission~\footnote{The design flow of a reflection unit cell is similar to transmission unit cell, which is detailed in Appendix.~\ref{}} unit cell design as a three-step logic:
(1) \textbf{Decomposition}, where the unit cell is segmented into discrete primitives (e.g., ducts, necks, cavities); (2) \textbf{Topology Parsing}, which hierarchically separates the structure into side-branch resonators and the main propagation path;  (3) \textbf{Response Prediction}, where complex branches are reduced to equivalent impedances and integrated into a global transfer matrix chain, and then computes transmittance and phase shift rapidly.

\sssec{Acoustic Primitive Decomposition.} First, \sysname decomposes the continuous geometry of a unit cell into a sequence of discrete primitives (e.g., \textit{Neck, Cavity, Duct}). We categorize these primitives into two physical models based on their wave propagation characteristics under fluid density $\rho_0$ and sound speed $c_0$:

\begin{itemize}[leftmargin=10pt,topsep=0pt]
	\item \textit{Lumped Elements (Equivalent Circuits):} 
	For deep sub-wavelength components acting as localized reactive loads (e.g., the \textit{neck} and \textit{cavity} of a side-branch Helmholtz resonator), we employ \textit{Equivalent Circuit Models}. 
	A narrow \textit{neck} constricts flow, behaving as an acoustic mass (\textit{Inductor}, $Z_{neck} \approx j\omega \rho_0 l_{neck}/S_{neck}$). 
	A wide \textit{cavity} stores potential energy, behaving as an acoustic compliance (\textit{Capacitor}, $Z_{cav} \approx 1 / (j\omega C_a)$ , where $C_a = V_{cav}/\rho_0 c_0^2$ ). Here, $V_{cav}$ denotes the volume of the cavity. 
	
	\item \textit{Distributed Elements (Transmission Lines):} 
	Components where wave propagation effects are non-negligible are modeled as \textit{Transmission Lines}. This category mainly includes \textit{ducts} that carrying main wave propagation. Notably, a common space-coiling (zig-zag) structure is mathematically "unfolded" into an equivalent straight transmission line with an effective length $l_{eff}$ equal to the total path length. They are characterized by a characteristic impedance $Z_c = \rho_0 c_0 / S$ and wavenumber $k=\omega/c_0$.
	The impedance transforming for a duct is calculated as $Z_{duct} = -j Z_c \cot(kl_{eff})$.
	
	%	encompasses not only the main waveguides but also space-coiling (zig-zag) structures and wide chambers along the propagation path. Regardless of their geometric length, these elements are characterized by a wavenumber $k=\omega/c_0$ and characteristic impedance $Z_c = \rho_0 c_0 / S$. This modeling explicitly captures the impedance transformation and the spatial phase accumulation $\phi = k l$ critical for wavefront engineering.
\end{itemize}

%\begin{packeditemize}
%	\item \textbf{Distributed Elements:} For components like main ducts whose length is comparable to wavelength, we model them as \textit{Transmission Lines}. These components introduce phase delays and impedance transformation. For a duct of length $l$ and cross-sectional area $S$, the characteristic impedance is $Z_c = \rho_0 c_0 / S$ and the wavenumber is $k = \omega/c_0$.
%	
%	\item \textbf{Lumped Elements:} For sub-wavelength components like narrow necks and expanded cavities, we employ \textit{Equivalent Circuit Models}.  A narrow neck constricts flow, behaving as an acoustic mass (\textit{Inductor}, $Z_{neck} \approx j\omega \rho_0 l_{eff}/S_{neck}$). A cavity stores potential energy, behaving as an acoustic compliance (\textit{Capacitor}, $Z_{cav} \approx 1 / (j\omega C_a)$). 
%\end{packeditemize}
\sssec{Hierarchical Topology Relationships.} 
Acoustic primitives are connected via specific topological connections to form a functional unit cell. To handle complexity, our solver distinguishes between two hierarchical levels as follows: 

\underline{\textit{1) Side-branch Topology (Impedance Domain):}} This level defines the localized connectivity within a resonant structure attached to the main path (e.g., a Helmholtz resonator). The goal is to reduce the entire branch into a single scalar input impedance $Z_b$ using circuit equivalence rules:

\begin{itemize}[leftmargin=10pt,topsep=0pt]
	\item \textit{Series Composition}: If the sound stream travels in only one direction, the components are effectively in series (e.g., a single Helmholtz resonator where a \textit{Neck} is followed by a \textit{Cavity}.) The total impedance is the sum of individual impedances $Z_b = \sum Z_{i}, Z_{i}\in (Z_{neck},Z_{cav}, Z_{duct})$ 
	
	\item \textit{Parallel Composition}: If a branch splits into multiple sub-paths (e.g., a cascaded resonator), the total impedance can be derived as  $Z_b = 1/\sum \frac{1}{Z_i}, Z_{i}\in (Z_{neck},Z_{cav}, Z_{duct})$  
\end{itemize}

Notably,it's possible for both series and parallel composition to occur simultaneously within a branch structure, as shown in Fig.~\ref{}. By employing a recursive solver, \sysname reduces nested resonator into a single impedance $Z_b$. 

\underline{\textit{\textit{2) Main Path Topology (Matrix Domain):}}} This level defines the global propagation from the unit cell inlet to the outlet, typically with parallel surfaces. We handle two fundamental connection types by typically formulating a $2\times2$ transfer matrix based on Transfer Matrix Method (TMM), representing the upstream and downstream at each cross-section. 

\begin{itemize}[leftmargin=10pt,topsep=0pt]
	\item \textit{Shunt Connection:} 
	A side-branch structure act as a parallel load attached to the main path. This creates a discontinuity modeled by inserting a \textit{Shunt Matrix} into the main chain $\mathbf{M}_{shunt} = \begin{bmatrix} 1 & 0 \\ 1/Z_b & 1 \end{bmatrix}$,
	%	\begin{equation}
<<<<<<< HEAD
	%		\mathbf{M}_{shunt} = \begin{bmatrix} 1 & 0 \\ 1/Z_b & 1 \end{bmatrix}
	%	\end{equation}
=======
		%		\mathbf{M}_{shunt} = \begin{bmatrix} 1 & 0 \\ 1/Z_b & 1 \end{bmatrix}
		%	\end{equation}
>>>>>>> 49294a80e92cbd25c5b1529c159ff831200efa5e
	where $Z_b$ is the total input impedance looking into the side structure.
	
	\item \textit{Series Connection}: Any component aligned with the main propagation axis (commonly is a duct), allows the wave to transmit through it. This is modeled as a \textit{Series Matrix} that captures phase delay and impedance transformation $\mathbf{M}_{series} = \begin{bmatrix} \cos(kl) & j Z_c \sin(kl) \\ \frac{j}{Z_c}\sin(kl) & \cos(kl) \end{bmatrix}$.
	%	\begin{equation}
<<<<<<< HEAD
	%		\mathbf{M}_{series} = \begin{bmatrix} \cos(kl) & j Z_c \sin(kl) \\ \frac{j}{Z_c}\sin(kl) & \cos(kl) \end{bmatrix}
	%	\end{equation}
=======
		%		\mathbf{M}_{series} = \begin{bmatrix} \cos(kl) & j Z_c \sin(kl) \\ \frac{j}{Z_c}\sin(kl) & \cos(kl) \end{bmatrix}
		%	\end{equation}
>>>>>>> 49294a80e92cbd25c5b1529c159ff831200efa5e
\end{itemize}



%To capture the complex interactions within the metasurface, we formulate the system using the Transfer Matrix Method. The acoustic state is described by the pressure-velocity vector $\mathbf{V} = [p, U]^T$. Our solver distinguishes between the \textbf{Main Propagation Path}, where transfer matrices are cascaded, and the \textbf{Side Branches}, where impedances are aggregated via equivalent circuit rules.


\sssec{Global Response Calculation.} The final step integrates these components to predict the spectral response. By traversing the main path \textbf{from inlet to outlet}, the global transfer matrix $\mathbf{M}$ is constructed by cascading the individual matrices: $\mathbf{M} = \prod \mathbf{M}_i = \begin{bmatrix} M_{11} & M_{12} \\ M_{21} & M_{22} \end{bmatrix}$, where $\mathbf{M}_i \in \{\mathbf{M}_{shunt}, \mathbf{M}_{series}\}$. We apply boundary conditions assuming an anechoic termination with characteristic impedance $Z_0 = \rho_0 c_0 / S_0$, where $S_0$ is the input port area. The complex transmission coefficient is derived from the elements of the global matrix:
\begin{equation}
<<<<<<< HEAD
t = \frac{2 Z_0}{M_{11} Z_0 + M_{12} + M_{21} Z_0^2 + M_{22} Z_0} \nonumber
\end{equation}
Finally, the target acoustic responses, \textbf{Transmittance} $T$ and \textbf{Phase Shift} $\phi$, are computed as: $T = |t|^2, \phi = \arg(t)$, respectively. This formulation enables \sysname to transfer the original FEM simulations into cascaded matrix computation, accelerating spectral response prediction. 
=======
	t = \frac{2 Z_0}{M_{11} Z_0 + M_{12} + M_{21} Z_0^2 + M_{22} Z_0} \nonumber
\end{equation}
Finally, the target acoustic responses, \textbf{Transmittance} $T$ and \textbf{Phase Shift} $\phi$, are computed as: $T = |t|^2, \phi = \arg(t)$, respectively. This formulation enables \sysname to transfer the original FEM simulations into cascaded matrix computation, accelerating spectral response prediction.

>>>>>>> 49294a80e92cbd25c5b1529c159ff831200efa5e

%While calculating the required spatial profiles is theoretically straightforward, realizing physical unit cells that precisely match these complex amplitude and phase requirements represents the primary bottleneck in AMS development. This challenge is further exacerbated in broadband applications where material dispersion becomes significant.




%\subsection{Modeling Acoustic Structure}
%Common acoustic response calculation relies on finite element method (FEM) simulations. While FEM is accurate, it is computationally expensive and time-consuming, often requires several minutes for each simulation. In order to accelerate the dataset construction, we introduce the lumped parameter models~\cite{} and incorporate it with transfer matrix method~\cite{}.
%
%\sssec{Discrete Components Modeling.} Instead of viewing acoustic structure as a holistic structure, \sysname decomposes complex acoustic structures into discrete acoustic primitives (Neck, Cavity, Duct). In the sub-wavelength regime, such acoustic components can be modeled as "lumped" elements~\footnote{The dimensions of the lumped element is much smaller than the wavelength.} Based on the concept of equivalent circuits~\cite{}, this analogy maps sound pressure to voltage and volume velocity to current , thus making acoustic impedance equivalent to the impedance of components in a circuit. Specifically, this abstraction decomposes unit cells into fundamental building blocks with distinct electrical behaviors:
%\begin{packeditemize}
%    \item \textbf{Acoustic Mass (Inductance):} A narrow duct or neck constricts flow, resisting acceleration. This behaves like an inductor $L_a \approx \rho l_{eff}/S$, where $\rho$ is density, $S$ is area, and $l_{eff}$ is effective length.
%	\item \textbf{Acoustic Compliance (Capacitance):} A large cavity stores potential energy via compression. This behaves like a capacitor $C_a \approx V_{cav}/\rho c^2$, where $V_{cav}$ is the volume and $c$ is sound speed.
%	\item \textbf{Transmission Line (Duct):} A uniform waveguide where wave propagation is significant. It introduces phase delay and transforms impedance, analogous to an electrical transmission line with characteristic impedance $Z_c = \rho c / S$ and propagation constant $k = \omega/c$.
%\end{packeditemize}
%
%
%\sssec{Transfer Matrix Model.} Next, we consider the transmission of acoustic energy through structures, using a transfer matrix model to capture the flow of sound across multiple components. This model is particularly effective for representing cascaded systems of acoustic components. In our approach, each component is represented by a $2\times2$ transfer matrix $\mathbf{T}$, which links the incident and outgoing pressure and velocity:
%\begin{equation}
%	\begin{bmatrix} p_{in} \\ U_{in} \end{bmatrix} = \mathbf{T} \begin{bmatrix} p_{out} \\ U_{out} \end{bmatrix} = \begin{bmatrix} A & B \\ C & D \end{bmatrix} \begin{bmatrix} p_{out} \\ U_{out} \end{bmatrix}
%\end{equation}
%For a system of $N$ cascaded components, the total transfer matrix $\mathbf{T}_{total}$ is simply the product of individual matrices: $\mathbf{T}_{total} = \prod_{i=1}^{N} \mathbf{T}_i$.
%Key acoustic properties, such as the transmission coefficient $t$, are then derived from the global matrix elements:
%\begin{equation}
%	t = \frac{2 Z_0}{A_{tot} Z_0 + B_{tot} + C_{tot} Z_0^2 + D_{tot} Z_0}
%\end{equation}
%where $Z_0$ is the characteristic impedance of the medium. This formalism not only provides a rapid forward solver (milliseconds vs. minutes for FEM) but also establishes the structural "grammar" for our generative model: a valid unit cell is a sequence of impedance-matched circuit components.



==> intro.tex <==
% !TEX root = main.tex
\section{Introduction}
Acoustic metamaterials (AMM)~\cite{fok2008acoustic} are artificially engineered sub-wavelength structures composed of cavities, ducts, or coils much smaller than the sound wavelength, which exhibit extraordinary acoustic properties to manipulate the amplitude and phase, driving applications such as sound absorption~\cite{Ma2014NatMater,LiAssouar2016APL,li2023sound,yang2022development}, enhancement~\cite{zhang2021remote,ning2025portable}, and voice assistant defense~\cite{lloyd2023mitigating,ning2025metaguardian}. By strategically arranging these metamaterial bricks into planar arrays, acoustic metasurfaces (AMS)~\cite{Assouar2018NRM} are constructed to achieve fine-grained sound wave control such as focusing~\cite{li2015metascreen,qi2018ultrathin,lu2023achromatic,chen2018broadband,zhu2021nonlocal} and reflection~\cite{Li2013SciRep,Li2014PRApp,Xie2014NatCommun,Tang2014SciRep}. While initial studies focused on narrow-band behaviors, emerging applications increasingly demand broadband capabilities (e.g., broadband noise reduction~\cite{guo2023phase,ryoo2022broadband}, directional speaker~\cite{li2024mudis}, achromatic focusing for clinical therapy~\cite{tang2021broadband,lu2023achromatic}, imaging~\cite{fu2024adaptive} and beam steering for communication~\cite{xie2014wavefront,Zhang2023NSDIAMS}). Realizing these functionalities requires meticulously designing metamaterial structures to match target acoustic response profiles (i.e., amplitude and phase), which is challenged by the dispersive nature of acoustics~\cite{bruneau2013fundamentals}: the intrinsic frequency-coupling of amplitude and phase complicates the effort to maintain accurate response profiles across a wide spectrum.

 


%Acoustic metasurfaces (AMS), typically composed of numerous sub-wavelength unit cell structures, enable fine-grained control over incident sound waves by modulating the amplitude and phase response at each cell location. By arranging these cells strategically, AMS can realize typical sound wave manipulation such as acoustic focusing~\cite{li2015metascreen,qi2018ultrathin,lu2023achromatic,chen2018broadband}, reflection~\cite{Li2013SciRep,Li2014PRApp,Xie2014NatCommun,Tang2014SciRep}, and sound absorption~\cite{Ma2014NatMater,LiAssouar2016APL,zhu2021nonlocal}.  While early research primarily targeted single-frequency behaviors, many practical applications increasingly require broadband performance (e.g., broadband noise reduction~\cite{guo2023phase,ryoo2022broadband}, directional speaker~\cite{li2024mudis}, achromatic focusing for clinical therapy~\cite{tang2021broadband,lu2023achromatic}, super-resolution imaging~\cite{fu2024adaptive} and beam steering for communication~\cite{xie2014wavefront,Zhang2023NSDIAMS}).  This imposes challenges in designing unit cells that maintain precise response profiles across a broad frequency due to 
%the dispersive nature of acoustic structures~\cite{bruneau2013fundamentals}: the amplitude and phase responses are intrinsically coupled with frequency.

%Acoustic metasurfaces (AMS)~\cite{}, typically composed of numerous sub-wavelength cell structures, have attracted significant attention recently due to easy fabrication and exceptional capability to manipulate sound waves. AMS manipulates incident acoustic waves by independently modulating the phase and amplitude at each unit cell position. Through the stragetic arrangement of the unit cells, AMS can potentially enable immense applications such as noise absorption~\cite{}, acoustic focusing~\cite{}, and super-resolution imaging~\cite{}.   
%
%The performance of AMS is fundamentally determined by the microscopic design of its constituent unit cells. While early research~\cite{} primarily on single-frequency response, real-world applications increasingly demand wideband functionality to handle complex acoustic applications, such as broadband noise reduction~\cite{} or multi-frequency sensing and communication~\cite{}. Designing unit cells that maintain precise phase and amplitude profiles across a broad frequency range introduces a significant challenge due to the dispersive nature of acoustic structures~\cite{}, where the amplitude and phased responses are intrinsically coupled with frequency.

Existing approaches for acoustic metamaterial design face several limitations. Heuristic workflows~\cite{BendsoeSigmund2004TOBook,Molesky2018NatPhotonInverseDesign} and traditional optimizations(e.g., gradient descent~\cite{jensen2011topology,AppliedAcoustics2023TOAMS,noguchi2021topology} or genetic algorithms~\cite{jafar2018adaptive,johnson1997genetic,Li2012JASAGA}) require manual objective, and are hindered by slow iterations and local minima. While data-driven regressors~\cite{Zhang2023ActaMechSinInverseAcoustic,Lv2024MaterialsAcousticMetasurfaceDL,Zhou2025SciRepBroadbandAbsDL,Zhu2025ActaAcusticaANNAbsorber,AppliedAcoustics2025CylPlateDL,AppliedAcoustics2026NewInvDL,JSV2025InvDL118789} accelerate inference, they are also restricted to pre-defined templates. Any change in the search space requires regenerating the massive training dataset, limiting topological flexibility. 

%Since data acquisition commonly relies on computationally expensive finite element methods (FEM), this topological inflexibility limits agile design iterations.

Recently, while image-based generative models have shown promise in electromagnetic domain~\cite{an2021multifunctional,zhao2025metagen}, their application in acoustics~\cite{Amirkulova2022ICA} remains scarce. Directly adopting pixel-based paradigms to acoustics is non-trivial: (i) Projecting continuous dimensions onto discrete pixel grids introduces quantization errors; since acoustic resonances are highly sensitive to dimension perturbations, this severely compromises physical fidelity. (ii) Acoustic wave propagation strictly relies on structural continuity; however, image-based models may generate topological disconnections such as broken isolating islands, rendering physically unrealizable. Therefore, there still remains a gap in acoustic metamaterial design, which can \textit{accommodate varying topologies while intrinsically ensuring structural continuity and physical fidelity.}



%Despite the importance of unit cell inverse design, existing approaches face several limitations. Early approaches~\cite{} mainly based on empirical heuristics and professional expertise, involving tedious and inefficient trial-and-error iterations. Subsequently, parameterized optimization methods~\cite{} were introduced to search  within a pre-defined parameter space. Traditional optimizations~\cite{} like gradient descent or genetic algorithms often require manual optimization objectives and are prone to getting trapped in local minima. Recent advances in neural network-based inverse design~\cite{} utilize parameter regression for rapid inference. However, these data-centric models are typically confined to fixed geometric topologies. Any change in parameter searching space requires regenerating the entire dataset and retraining the model, severely limiting design flexibility. More importantly, these approaches still depend on pre-defined templates, relying heavily on expert intuition. Furthermore, while some works~\cite{} have explored image generative models for metasurface pattern design, these efforts are restricted to the electromagnetic domain and remain unexplored in acoustics.  This is primarily due to the unique challenges of acoustic physics: generating training data via Finite Element Method (FEM) simulations is computationally prohibitive, and pixel-based generation often fails to enforce the strict geometric connectivity required for acoustic unit cells. 

To bridge this gap, we propose \sysname, a novel sequence-based physical generative framework for acoustic metamaterial design given a target spectrum response. We fundamentally reconceptualize the design problem: instead of treating the structures as an static image or a parameterize template, we view it as a structured sequence of compositional acoustic primitives (e.g., \textit{Duct, Neck, Cavity}), together with their topological relations  (e.g., \textit{Series, Shunt}) and continuous geometric parameters (e.g., \textit{Width, Height}). This paradigm, which redefines inverse design as a sequence-to-sequence (Seq2Seq) translation task, is motivated by several core insights: (i) The sequence formulation maintains alignment with the physics of acoustic wave propagation, naturally mirroring the continuous cascade of transmission events as sound wave traverses distinct structural elements and ensuring continuity; (ii) The structural complexity (i.e., sequence length) can be flexibly adjusted to match target spectrum response, without being limited to a specific template.  (iii) The structured sequence provides a clear semantic description, which carries accurate physical meaning (e.g., numerical geometric dimension) and is directly editable. Specifically, the realization of \sysname encompasses three innovations as below: 


%To address these challenges, we propose \sysname, a physical-enhanced generative framework for scalable and accurate inverse design of acoustic metasurface elements using equivalent-circuit modeling~\cite{}. We fundamentally reconceptualize the design problem: instead of treating the structures as an image or a fixed set of template parameters, we view it as a sequence of compositional acoustic primitives (e.g., \textit{Duct, Neck, Cavity}), together with their topological relations  (e.g., \textit{Series, Shunt}) and continuous geometric parameters (e.g., \textit{Width, Height}). Under this formulation, inverse design becomes a sequence-to-sequence (Seq2Seq) translation task: given a target frequency response, the model generates a structured description of the unit cell, as depicted in Fig.~\ref{}. Compared to pattern-based generative approaches~\cite{}, \sysname offers two advantages: Firstly, \sysname outputs precise numerical values, eliminating discretization errors during image-to-structure conversion. Secondly, the structured text output is editable and interpretable, making subsequent optimization or manual adjustments feasible. \yj{Motivate from the broadband/complex design and the seq2seq task}

%To bridge this gap, in this paper, we propose \sysname, a novel Generative Framework for scalable and accurate inverse design of acoustic metasurface unit cell based on equivalent circuit theory~\cite{}. We fundamentally reconceptualize the design problem: instead of treating the structures as image with fixed-pixel resolutions or a fixed parameter set within pre-defined templates, we view it as a sequence of discrete, minimum acoustic components (e.g., \textit{Duct, Neck, Cavity}). As depicted in Fig.~\ref{}, our proposed \sysname framework contains two parts: \textit{a) Rapid massive dataset construction:} We specifically define a tokenizer including discrete acoustic structure, structural relationships, and their geometric values, and implement a Physics recursive solver to calculate response by mapping these discrete components to electrical equivalents (i.e., resistors, capacitors, inductors). This obtains XXx faster generation than finite element method (FEM)-based generation. \textit{b) tranformer-based generative model:} we formulate the inverse design task as a sequence-to-sequence (Seq2Seq) translation problem, where a target acoustic response is translated into a sequence of text including pre-defined tokens. Comparing to diffusion-based pattern generation approaches, \sysname offers two advantages: Firstly, \sysname outputs precise numerical values, eliminating discretization errors during image-to-structure conversion. Secondly, the structured text output is editable and interpretable, making subsequent optimization or manual adjustments feasible.

\sssec{\sysname Language Definition.}
As a first step, \sysname must represent a geometric structure as a 1D sequence suitable for generative models. A naive linear serialization fails to preserve critical topological information, such as  main propagation path versus side-branch hierarchies, or series/shunt connectivity. To address this, we formalize the inverse design into a domain-specific language (DSL) that jointly represents discrete structural logic and geometric parameters. Specifically, the DSL consists of a tailored \textbf{vocabulary} of discrete symbols, including \emph{structure tokens} representing acoustic primitives (e.g., \texttt{[DUCT]}, \texttt{[CAVITY]}) and \emph{relationship tokens} acting as delimiters to encode topological hierarchy and branch connectivity (e.g., \texttt{[SHUNT\_START]},\texttt{[SHUNT\_END]}). In addition to these discrete symbols, each structure is associated with a set of continuous geometry parameters that specify its dimensions. To assemble these elements into valid sequences, we design a \textbf{grammar} based on a depth-first traversal (DFT) strategy, which linearizes the acoustic tree along the wave-propagation direction. The grammar requires each structure token to be paired with its corresponding geometry parameter fields, ensuring semantic consistency between topology and dimensions. Finally, we impose explicit \textbf{constraints} to guarantee structural integrity and physical realizability, including topological constraints (e.g., non-empty branches) and geometric constraints (e.g., sub-wavelength bounds and spatial non-overlap). We further implement a \textbf{validity checker} to verify whether a sequence satisfies all grammar and constraint rules, which is used in both the dataset generation and inference phases.

\sssec{High-Fidelity Dataset Construction.}
Once the language is defined, \sysname constructs a large-scale training dataset of valid structural sequences and their corresponding acoustic responses. This poses two challenges:

\noindent\textit{1) Distribution bias.}
A naive strategy randomly assembles structures and geometric parameters. However, since the validity checker rejects spatial overlaps and illegal configurations, longer and more complex sequences are filtered out at higher rates, yielding a dataset biased toward trivial topologies. To mitigate this bias, \sysname employs a \textbf{complexity-balanced sampling strategy} that maintains an approximately uniform distribution over structural length, guaranteeing diverse topological coverage.

\noindent\textit{2) Precision gap.}
Obtaining high-fidelity acoustic responses at scale is computationally challenging. Mapping the sequence back to an image and using Finite Element Method (FEM) simulation (e.g., COMSOL) is computational prohibitive (3 s/sample), whereas analytical solver such as Transfer Matrix Method (TMM)~\cite{herrero2019matrix} is efficient but suffers from non-negligible errors ($0.116$ average MSE\footnote{MSE is defined as the mean squared error between the predicted response and the COMSOL ground truth.}) in multi-component structures due to scattering at cross-sectional discontinuities. This issue becomes more severe for complex topologies under our various complex topologies. To resolve this, we introduce an \textbf{efficient FEM-intervened correction mechanism} that models such errors as geometry-dependent equivalent-length corrections. With only a small pilot set of FEM simulations for calibration, the corrected physical solver retains analytical efficiency (0.024 s/sample) while achieving high fidelity ($0.011$ average MSE).


%\sssec{High-Fidelity Dataset Construction.} Once the language is established, \sysname must generate a massive training dataset pairing valid structural sequences with corresponding acoustic responses, which confronts two challenges:
%
%\noindent\textit{ 1) Distribution bias.} A strawman generation approach is to randomly assemble structures and parameters, but this suffers from severe distribution bias, Since our validity checker strictly discards spatial overlaps and illegal configurations, complex and long sequences are rejected at much higher rates, yielding a dataset heavily skewed toward simple, short topologies. To prevent overfitting to trivial cases, \sysname introduces a \textbf{complexity-balanced sampling strategy} that enforces a uniform distribution across structural lengths, guaranteeing diverse topological coverage.  
%
%\noindent\textit{ 2) Precision gap.} Next, \sysname needs to acquire ground-truth acoustic responses for massive dataset. Mapping the sequence back to an image and then use the traditional Finite Element Method (FEM) simulators (e.g., COMSOL) imposes intractable computational bottleneck (3s/sample). While analytical physical solver like the Transfer Matrix Method (TMM)~\cite{herrero2019matrix} offer milliseconds-level predictions, they suffer from precision loss ($0.116$ average MSE~\footnote{MSE is defined as mean square error between the predict response and the ground truth response calculated by COMSOL.}) in multi-component structures due to scattering at cross-sectional discontinuities, even more severe under our various complex topologies. To resolve this, we propose an \textbf{efficient FEM-intervened correction mechanism}. Based on the insight that these analytical errors are predominantly localized at cross-sectional junctions, we model the discrepancies as geometry-dependent equivalent length corrections. By calibrating these correction factors using a minimal pilot set of FEM simulations, our physical solver retains the ultra-fast efficiency (0.024s/sample) of analytical models while achieving high fidelity ($0.011$ average MSE).


%\sssec{High-Fidelity Dataset Construction.} The success of generative model depends on a large-scale, high-quality dataset. Traditional ground truth acquisition relies on FEM simulators (e.g., COMSOL), which are computationally expensive (taking minutes per sample), making the generation of massive dataset near impossible.  In comparison, equivalent-circuit approaches such as Transfer Matrix Method (TMM) provide milliseconds-level computation to obtain the propagation of acoustic waves.  However, standard TMM becomes inaccurate in multi-component geometries due to scattering and mode effects at cross-sectional discontinuities and junctions~\cite{}. 
%To address this issue, \sysname introduces a \textbf{physics-enhanced TMM} calibrated with minimal simulator data.  Our key insight is that most errors are localized at the cross-sectional discontinuities. These inaccuracies can be modeled as equivalent length corrections derived from the junction geometry. Instead of running full-wave simulations for every sample, we learned these correction factors using a minimal set of FEM data on basic connection units. By integrating this correction, \sysname retains TMM's efficiency while achieving accuracy comparable to full-wave FEM (MSE <XXX). This physical solver enables the rapid construction of a massive, topologically diverse dataset, containing varied structural descriptions and their corresponding responses.
  
%\sssec{High-Fidelity Massive Dataset Construction.} The success of generative model depends on a large-scale, high-quality dataset. Traditional ground truth acquisition relies on FEM using simulators (e.g., COMSOL), which are computationally expensive (taking minutes per sample), making the generation of massive dataset near impossible.  In comparison, equivalent circuit-based Transfer Matrix Method (TMM) offers milliseconds-level computation to obtain the propagation of acoustic waves through a composite structure.  However, it fails to capture complex scattering behavior~\cite{} of the sound wave transmission at junctions, leading to inaccuracies in multi-component geometries.   To address this issue, we introduce a  \textbf{physics-enhanced TMM} calibrated with minimal simulator data.  Our key insight is that the errors in standard TMM are localized at the cross-sectional discontinuities. These inaccuracies can be modeled as an equivalent length corrections derived from the junction geometry. Instead of running full-wave simulations for every sample, we extract these correction factors using a minimal set of FEM data on basic connection units. By integrating this correction, we achieve accuracy comparable to full-wave FEM (MSE <XXX) while maintaining millisecond-level inference speeds. This solver enables the rapid construction of a massive, topologically diverse dataset.

\sssec{Generative Framework for Inverse Design.} Traditional image-based frameworks~\cite{an2021multifunctional,zhao2025metagen,Amirkulova2022ICA} suffer from pixelation errors and topological disconnections. Furthermore, standard supervised learning struggles with the intrinsically ill-posed nature of acoustic inverse design, where multiple distinct structures can yield the identical target response. However, producing diverse yet valid structural candidates for a single acoustic target is practically important for accommodating varying manufacturing and spatial constraints. 
 

To address this, \sysname adopts a generative framework including a supervised pretraining followed by reinforcement learning (RL) finetuning. The \textbf{supervised pretrained model} is necessary for providing a stable prior for structural grammar and geometric validity. We then perform \textbf{RL fine-tuning} to unlock diverse solution exploration in physical response space. Moreover, the generated sequence of \sysname must remain physically realizable while producing multiple candidates. Specifically, Realizing this framework requires addressing three key challenges:

%learns the conditional mapping from target responses to structural sequences, providing a stable initialization and a strong prior for topology prediction, parameter regression, and sequence validity. This stage is necessary because direct RL from scratch in the hybrid discrete-continuous design space would be highly unstable and sample-inefficient. We then perform \textbf{RL fine-tuning} to enable one-to-many optimization in the physical response space. \sysname must satisfy two key requirements: (i) generate multiple candidates with diverse topologies for the same target response; and (ii) ensure that the generated sequences remain physically realizable.

\noindent\textit{1) Hybrid Modality Prediction.} The output sequence tightly couples discrete topology tokens and continuous geometric parameters. To prevent semantic misalignment, \sysname employs a \textbf{dual-head Transformer decoder} with a per-token parameter head, ensuring dimensional regression perfectly aligns with discrete structural decisions.

\noindent\textit{2) Geometry Constraints.} Generated sequences must strictly satisfy dimensional bounds, spatial non-overlap, and grammar rules. \sysname enforces these through a \textbf{structure-aware scalar reweighting mechanism} during pretraining, combined with explicit structural and overlap penalties during RL to restrict generation to physically realizable spaces.

\noindent\textit{3) One-to-Many Optimization via RL.} Supervised pretraining provides a stable, valid initialization but inherits deterministic sample-fitting biases. To unlock diverse topologies, \sysname leverages \textbf{RL fine-tuning} to optimize directly in the physical response space. Guided by a fast proxy or our physics-based solver , the policy actively explores the design space to discover high-fidelity, alternative solutions missed by exact parameter matching.






%\sssec{Generative Framework for Inverse Design.} Traditional image-based generative frameworks~\cite{} suffers from discretization errors when mapping continuous numerical values to fixed pixel grid. In contrast, based on above scalable dataset, \sysname treats the inverse design as a sequence-to-sequence translation task, mapping target acoustic responses directly to explicit geometric sequence descriptions (i.e., structure types, relationships, and dimensions). Specifically, realizing \sysname tackles two modeling challenges: 

%\sssec{Physics-Driven Inverse Framework.} Existing deep learning approaches for inverse design mainly rely on pixel-based generative models (e.g., GAN~\cite{} or Diffusion model~\cite{}). However, this "image-to-structure" conversion suffers from discretization errors when mapping continuous numerical values to fixed pixel grid. In contrast, distinct from pixel-wise generation, \sysname treats the unit cell design as a sequence-to-sequence translation task, mapping target acoustic responses directly to explicit geometric components (i.e., structure types, arrangement, and dimensions). However, realizing \sysname tackles two modeling challenges:
 
%\noindent\textit{ 1) "one-to-many" mapping challenge.}  The inverse design of an unit cell design is intrinsically an ill-posed problem: multiple distinct geometries can realize similar target responses. Traditional supervised training, which forces the model to memorize a specific ground truth for a given target, often causes confusions in multiple feasible solutions. To address this non-uniqueness challenge, we adopt a \textbf{forward-inverse tandem architecture}: By attaching pre-trained \textit{forward physical proxy model} to the generator, optimization can perform in the physical response space rather than forcing an exact match in the parameter space, thus allowing diverse and expansive design solutions. 

%Instead of minimizing the differences in the parameter space from a reference sample, we attach a pre-trained \textit{forward physical proxy model} to the generator. This allows the optimization objective to shift from the parameter space to the physical-informed response space, which enables the diverse and expansive design space of the model.

%\noindent\textit{ 2) Hybrid modality prediction.}  Unlike standard NLP tasks, the output of \sysname is hybrid including both discrete structure tokens (component types, relationships) and numerical geometry (dimensional values). These two modalities are tightly coupled, where the semantic meaning of a dimension depends entirely on the token type.  To handle this,  \sysname develops a \textbf{dual-head transformer decoder}, which features two parallel prediction heads: one classifies the discrete component tokens, while the other regresses their corresponding continuous numerical values. In conjunction with the forward physical proxy model, \sysname can generate a complete sequence comprising both structural logic and precise parameters in a single inference pass. \yj{What is the specific design here to differentiate traditional NLP task?}

%\sysname requires simultaneous prediction of both discrete topology (component types) and numerical geometry (dimensional values). These two modalities are tightly coupled, where the physical meaning of a dimension depends entirely on the component type. To handle this,  \sysname develops a \textbf{Dual-Head Transformer Decoder}, which features two parallel prediction heads: one classifies the discrete component tokens, while the other regresses their corresponding continuous numerical values. By companion with the forward physical proxy model, \sysname can generate a complete sequence comprising both structural logic and precise parameters in a single inference pass.

%\sssec{Confronting Geometry Violation.} Accurate inverse inference alone does not guarantee manufacturable designs. A valid sequence must satisfy three critical constraints: \textit{1) Dimensional Boundaries}: all geometric parameters must fall within fabrication limits; \textit{2) Spatial Non-overlap}: components must not intersect or collide; and \textit{3) Syntactic Correctness}: the sequence of tokens should follow a valid grammar order.
%
%A naive approach to append these constraints would be to train a binary classifier on a static dataset comprising valid and invalid samples. However, it is impossible to exhaustively enumerate all possible violation patterns due to the unbounded and highly imbalanced invalid space. To overcome this challenge, \sysname achieves validity in two steps: First, during data construction, we implement a \textbf{geometric validation checker} that reconstructs 2D layouts from sequence descriptions and discards collisions and illegal configurations. This ensures every sample in the training set is a valid sequence. Second, during model training, \sysname further introduces an \textbf{iterative discriminator-guided pipeline}: invalid samples generated by the model are harvested as hard negatives to continually refine a geometry discriminator, which is then incorporated into the generator’s learning objective to penalize illegal outputs. This joint training process and active feedback loop allow the generator to progressively learn complex geometric constraints that are difficult to encode statically, ensuring the production of valid, fabrication-ready structures. \yj{Need update to new methodology}



%However, such stochastic generation can result in physically invalid configuration (e.g., structural geometry overlap). To guarantee sequence in dataset are all manufacturable, we implement a strict \textbf{geometric validation checker} by mapping the text-geometric parameters into 2D spatial coordinates to reconstruct the physical layout. An automated detection algorithm is then employed to identify and discard any invalid designs containing structural overlaps or collisions, ensuring that every sample represents a valid unit cell. This checker will also serve as a constraint mechanism within the following generative model to enforce the prediction of geomtric-reasonable results.

%\sssec{Confronting Geometry Violation.} Although the inverse model can effectively map acoustic responses to geometric sequences, the raw predictions do not inherently guarantee physical realizability. A valid design must strictly adhere to three critical constraints: (1) \textit{Dimensional Boundaries}: all geometric parameters must fall within fabrication limits; (2)\textit{ Spatial Non-overlap}: components must not physically intersect or collide; and (3) \textit{Syntactic Correctness}: the sequence of tokens must follow a valid topological order.
%
%A naive approach to appending these constraints would be to train a binary classifier on a static dataset comprising of valid and invalid samples. However, this is fundamentally flawed due to the extreme class imbalance and the unbounded nature of the invalid space.  The space of invalid configurations is extremely larger than valid ones and it is impossible to exhaustively enumerate all possible violation patterns for training.  To overcome this, we incorporate an \textbf{Iterative Discriminator-guided Training Pipeline} through an adversarial strategy. Specifically, we implement a joint training pipeline: In each training epoch, Tinvalid structures generated by the model are harvested as "hard negatives" to refine the geometric discriminator. This updated discriminator is then integrated into the inverse model's loss function to penalize non-physical outputs. This active feedback loop allows the generator to progressively learn complex geometric constraints that are difficult to encode statically, ensuring the production of valid, fabrication-ready structures.

%We implement \sysname as an end-to-end framework that takes a target response and outputs a valid structural sequence and corresponding layout. \sysname is validated against COMSOL simulations and benchmarked against diffusion based~\cite{zhao2025metagen}, supervised learning, and Nearest neighbor optimization baselines in terms of training efficiency, inference latency, and accuracy. We also demonstrate how the structured sequence representation enables semantic edits-potentially assisted by LLMs—highlighting the semantic interpretability and editability advantages over pixel-based representation. 

We implement \sysname as an end-to-end framework that maps a target response to a valid structural sequence and its corresponding layout. We validate \sysname against COMSOL simulations and compare it with diffusion-based~\cite{zhao2025metagen}, supervised, and nearest-neighbor optimization baselines in terms of training efficiency, inference latency, and accuracy. We further show that the structured sequence representation supports semantic editing, potentially assisted by LLMs, demonstrating superior interpretability and editability over pixel-based representations.

%We implement an end-to-end framework where users input a target response to automatically obtain the corresponding geometric sequence and patterns. The system is validated against COMSOL simulations and benchmarked against diffusion-based baselines~\cite{} in terms of training efficiency and accuracy. Furthermore, we demonstrate the integration of LLM to edit generated sequences, highlighting the \sysname's unique semantic interpretability and editability compared to pixel-based approaches. Our results show that:
\sssec{Results: } Our results show that:
\begin{packeditemize}
	\item \sysname achieves a reconstruction accuracy of XXX MSE compared to full-wave simulations.  
	
	\item Compared to diffusion-based baselines, \sysname reduces training time by XXX and inference latency by XXX, and improves accuracy by XXX.
\end{packeditemize}

\sssec{Contributions: }\sysname's core contributions include:

\begin{packeditemize}
	\item A novel generative framework that reformulates acoustic metamaterial design as a Seq2Seq translation task.

	\item A domain-specific language for acoustic metamaterial inverse design. 
	
	\item A corrected physical solver for efficient high-fidelity
	large-scale dataset construction.
	
	\item A generative framework including supervised pretraining and RL finetuning to resolve one-to-many inverse problem while guarantee the validity.
	
	\item Extensive evaluation with complex broadband tasks including absorption and focusing and showcase unique semantic interpretability through LLM-assisted structural editing.
\end{packeditemize}   



==> related.tex <==
% !TEX root = main.tex
\section{Related Work}
\subsection{Acoustic Metasurface Applications}
Acoustic metasurfaces (AMS)~\cite{Assouar2018NRM} enable fine-grained control of the reflected/transmitted wavefront by spatially modulating sub-wavelength unit cells~\cite{memoli2017metamaterial,memoli2019vari}. Early studies
demonstrated wavefront engineering to achieve acoustic reflection~\cite{Li2013SciRep,Li2014PRApp,Xie2014NatCommun,Tang2014SciRep}, sound absorption~\cite{Ma2014NatMater,LiAssouar2016APL},  acoustic focusing~\cite{li2015metascreen,qi2018ultrathin,tang2021broadband,lu2023achromatic,chen2018broadband}, and impedance matching for efficient cross-medium (e.g., water-air) sound transmission~\cite{Bok2018PRL}.

Beyond fundamental wave control, recent advances~\cite{jiang2025survey} have leveraged the cost-efficiency and fabrication ease of AMS to enhance acoustic sensing and communication systems. In the realm of sensing, optimized unit cell arrangements have been deployed for spatial perception~\cite{fu2024pushing}, high-precision indoor localization~\cite{wang2025metasonic}, and acoustic imaging~\cite{wang2025high}. Similarly, for communication, AMS serves as a passive component for beam steering~\cite{xie2014wavefront}, reflection re-focusing~\cite{li2014experimental}, and wavefront shaping in audio transmission~\cite{li2024mudis,zhou2025m2silent}. Notably, Zhang et al.~\cite{Zhang2023NSDIAMS} achieved long-range capabilities by integrating AMS with phased arrays. Furthermore, compact AMS designs have reduced system size and enable novel  applications, including lightweight direction recognition~\cite{bai2022spidr,garg2021owlet,yuan2025sonicsieve} and inaudible voice attacks and defense~\cite{ning2025portable,ning2025metaguardian}. However, the majority of these works are often restricted by the intrinsic narrowband resonance of the unit cells. Current research frontiers~\cite{tang2021broadband,lu2023achromatic,chen2018broadband,ning2025metaguardian, he2024cw} are gradually shifting towards broadband design to accommodate complex, multi-frequency needs.

\subsection{Metasurface Element Design}
\sssec{Optimization-based inverse design.} Conventional inverse design is typically formulated as an iterative parameter search over predefined templates, heavily relying on heuristic tuning and trial-and-error iterations~\cite{BendsoeSigmund2004TOBook,Molesky2018NatPhotonInverseDesign}. While automated strategies like Genetic Algorithms~\cite{jafar2018adaptive,johnson1997genetic,Li2012JASAGA} and gradient-based methods~\cite{jensen2011topology,AppliedAcoustics2023TOAMS,noguchi2021topology} improve upon manual heuristics, they remain computationally expensive and highly susceptible to local optima. Furthermore, these approaches require the manual definition of complex objective functions. As design requirements shift toward broadband or complex responses, the exponential expansion of the parameter space severely impedes convergence and makes defining robust objectives increasingly difficult.

\sssec{Data-driven supervised inverse design.} In recent years, deep learning has been extensively explored for inverse design, predominantly formulated as a supervised regression task mapping target responses to specific geometric parameters. This paradigm has been successfully applied to optimize various acoustic applications~\cite{Zhang2023ActaMechSinInverseAcoustic,Lv2024MaterialsAcousticMetasurfaceDL,Zhou2025SciRepBroadbandAbsDL,Zhu2025ActaAcusticaANNAbsorber,AppliedAcoustics2025CylPlateDL,AppliedAcoustics2026NewInvDL,JSV2025InvDL118789}. However, these models assume a fixed topology with a static, fixed-dimensional parameterization. Consequently, any modification to the design space (e.g., changing connectivity or adding components) requires massive data resampling and retraining, suffering from scalability bottlenecks.


% This paradigm has seen widespread success across nanophotonics~\cite{Liu2018ACSP,Peurifoy2018SciAdv,tahersima2019deep}, electromagnetics~\cite{Qiu2019AdvSci,ghorbani2021deep}, and acoustics~\cite{Zhang2023ActaMechSinInverseAcoustic,Lv2024MaterialsAcousticMetasurfaceDL,Zhou2025SciRepBroadbandAbsDL,Zhu2025ActaAcusticaANNAbsorber,AppliedAcoustics2025CylPlateDL,AppliedAcoustics2026NewInvDL,JSV2025InvDL118789}. However, these models assume a fixed topology with a static, fixed-dimensional parameterization. Consequently, any modification to the design space (e.g., changing connectivity or adding components) requires massive data resampling and retraining, suffering from scalability bottlenecks.


%By representing a unit cell as a \textbf{sequence} of acoustic primitives, topological relations, and continuous geometric values, \sysname expands the expressiveness of the design space and formulates inverse design as a Seq2Seq generation task.

\sssec{Generative inverse design.} To address the non-uniqueness of inverse design, generative models have been introduced to treat structural design as a conditional image generation task. Early frameworks utilized GANs~\cite{an2021multifunctional} and CVAEs~\cite{Yan2025YMSSP, Amirkulova2022ICA} to synthesize potential acoustic candidates within a latent space. Recent state-of-the-art methods~\cite{zhao2025metagen} employ diffusion to achieve high quality results, but diffusion-based methodologies haven't been seen in acoustic domain yet. However,  acoustic unit cells rely on intricate, connected voids and require manufacturability constraints (e.g., connectivity and printable supports). Free pixel generation often yield invalid topology such as disconnected channels, rendering generated samples unmanufacturable. Moreover, these pattern-based generative frameworks are based on a pixel paradigm, treating physical structures as bitmap images. This pixel-wise representation introduces quantization errors when converting continuous dimensions to discrete pixel grid. 




%Generative models~\cite{liu2018generative} are effective to handle non-uniqueness of inverse design, modeling the problem as structural images generation. While early works utilized GANs~\cite{an2021multifunctional,Wen2019arXiv,Jiang2019ACSNano,hodge2019multi,hodge2019rf} and CVAEs~\cite{Yan2025YMSSP,Amirkulova2022ICA,lin2022machine,tanriover2022deep} to synthesize potential structural candidates, recent state-of-the-art methods like  MetaGen~\cite{zhao2025metagen} employ diffusion to achieve higher quality results and a more stable training process. However, these pattern-based generative frameworks are based on a pixel paradigm, treating physical structures as bitmap images. This pixel-wise representation introduces quantization errors when converting continuous dimensions to discrete pixel grid. Moreover, unlike electromagnetic element design~\cite{zhao2025metagen}, acoustic unit cells rely on intricate, connected voids and require manufacturability constraints (e.g., connectivity and printable supports). Free pixel generation often yield invalid topology such as disconnected channels, rendering generated samples unmanufacturable. 

%\sssec{$\blacksquare$ Summary of Differences.}
%Existing methods are limited by the high computational cost of FEM data, the inflexibility of fixed templates, and the discretization errors inherent in pixel-based generation.
%\sysname overcomes these by: (1) leveraging a physics-enhanced TMM for rapid, high-fidelity data generation; (2) treating unit cells as continuous parametric sequences rather than discrete images; and (3) enforcing strict manufacturability via iterative discriminator guidance, ensuring every generated design is physically valid.

\sssec{$\blacksquare$ Summary of Differences.}
Overall, existing AMS element inverse design is commonly limited by: (1) expensive FEM data that hinders scalable generative training; (2) template rigidity that prevents structural exploration; (3) pixel-based generation that struggles with precision and manufacturable connectivity;
In contrast, \sysname overcome these by (1) leveraging a \textbf{physics-enhanced TMM} for rapid, high-fidelity data generation; (2) reformulating unit cells as \textbf{structured sequences} to allow flexible topological variation; (3) guaranteeing manufacturability through an \textbf{embedded geometry constraints mechanism}.

